BEval: A Plug-in to Extend Atelier B with Current Verification Technologies

This paper presents BEval, an extension of Atelier B to improve automation in the verification activities in the B method or Event-B. It combines a tool for managing and verifying software projects (Atelier B) and a model checker/animator (ProB) so that the verification conditions generated in the former are evaluated with the latter. In our experiments, the two main verification strategies (manual and automatic) showed significant improvement as ProB's evaluator proves complementary to Atelier B built-in provers. We conducted experiments with the B model of a micro-controller instruction set; several verification conditions, that we were not able to discharge automatically or manually with AtelierB's provers, were automatically verified using BEval.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{Nazareno Aguirre, Leila Ribeiro (Eds.):\\
First Latin American Workshop on Formal Methods (LAFM 2013)\\
EPTCS 139, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.139.5}{10.4204/EPTCS.139.5}}
\pdfoutput=1

